An explicit Euler scheme with strong rate of convergence for financial SDEs with non-Lipschitz coefficients

We consider the approximation of stochastic differential equations (SDEs) with non-Lipschitz drift or diffusion coefficients. We present a modified explicit Euler-Maruyama discretisation scheme that allows us to prove strong convergence, with a rate. Under some regularity and integrability conditions, we obtain the optimal strong error rate. We apply this scheme to SDEs widely used in the mathematical finance literature, including the Cox-Ingersoll-Ross~(CIR), the 3/2 and the Ait-Sahalia models, as well as a family of mean-reverting processes with locally smooth coefficients. We numerically illustrate the strong convergence of the scheme and demonstrate its efficiency in a multilevel Monte Carlo setting.

==> support_chaire.tex <==
presentation
\date{la date \\ \vspace{5mm} 
{\tiny The research of the author benefited from the support of
\\  the `Chaire Risque de cr\'edit', F\'ed\'eration Bancaire Fran\c caise. }}

article
\footnote{The research of the author benefited from the support of the `Chaire Risque de cr\'edit', F\'ed\'eration Bancaire Fran\c caise.}
